Online Learning: A Comprehensive Survey

Online learning represents an important family of machine learning algorithms, in which a learner attempts to resolve an online prediction (or any type of decision-making) task by learning a model/hypothesis from a sequence of data instances one at a time. The goal of online learning is to ensure that the online learner would make a sequence of accurate predictions (or correct decisions) given the knowledge of correct answers to previous prediction or learning tasks and possibly additional information. This is in contrast to many traditional batch learning or offline machine learning algorithms that are often designed to train a model in batch from a given collection of training data instances. This survey aims to provide a comprehensive survey of the online machine learning literatures through a systematic review of basic ideas and key principles and a proper categorization of different algorithms and techniques. Generally speaking, according to the learning type and the forms of feedback information, the existing online learning works can be classified into three major categories: (i) supervised online learning where full feedback information is always available, (ii) online learning with limited feedback, and (iii) unsupervised online learning where there is no feedback available. Due to space limitation, the survey will be mainly focused on the first category, but also briefly cover some basics of the other two categories. Finally, we also discuss some open issues and attempt to shed light on potential future research directions in this field.

==> prediction_expert_ol.tex <==

\subsection{Overview}
This is an important online learning subject \cite{roughgarden2017online} with many applications. A general setting is as follows. A learner has $N$ experts to choose from, denoted by integers $1,\dots,N$. At each time step $t$, the learner decides on a distribution $\p_t$ over the experts, where $p_{t,i}\ge 0$ is the weight of each expert $i$, and $\sum^N_{i=1}p_{t,i}=1$. Each expert $i$ then suffers some loss $\ell_{t,i}$ according to the environment. The overall loss suffered by the learner is $\sum^N_{i=1}p_{t,i}\ell_{t,i}=\p_t^\top\mathbf{\ell}_t$, i.e., the weighted average loss of the experts with respect to the distribution chosen by the learner.

Typically we assume that the loss suffered by any expert is bounded. More specifically, it is assumed that $\ell_{t,i}\in[0,1]$ without loss of generality. Besides this condition, no assumptions will be made on the form of the loss, or about the how they are generated. Suppose the cumulative losses experienced by each expert and the forecaster are calculated respectively as follows:
\bqs
L_{t,i}=\sum^t_{s=1}\ell_{s,i},\quad L_t=\sum^t_{s=1}\p_t^\top\mathbf{\ell}_t.
\eqs
The loss difference between the forecaster and the expert is known as the ``regret'', i.e.,
\bqs
R_{t,i} = L_t - L_{t,i},\quad i=1,\ldots,N.
\eqs
The goal of learning the forecaster is to make the regret with respect to each expert as small as possible, which is equivalent to minimizing the overall regret, i.e.,
\bqs
R_T=\max_{1\le i\le N} R_{T,i}=L_T-\min_{1\le i\le N} L_{T,i}
\eqs
In general, online prediction with expert advice is to design an ideal forecaster that can achieve a vanishing per-round regret, a property known as the Hannan consistency~\cite{citeulike:2683709}, i.e.,
\bqs
R_T = o(T) \Leftrightarrow \lim_{T\rightarrow\infty}\frac{1}{T}\left(L_T - \min_{1\le i\le N}L_{T,i}\right)
\eqs
%The above property is known as the Hannan consistency~\cite{citeulike:2683709}.
A learner achieving this is called a Hannan consistent forecaster~\cite{DBLP:books/daglib/0016248}.

\subsection{Weighted Majority Algorithms} The weighted majority algorithm (WM) is a simple but effective algorithm that makes a binary prediction based on a series of expert advices \cite{DBLP:journals/iandc/LittlestoneW94,littlestone1989weighted}. The simplest version is shown in Algorithm \ref{alg:wmm}, where $\beta \in (0,1)$ is a user specified discount rate parameter.
\begin{algorithm}[hptb]
\label{alg:wmm}
\caption{Weighted Majority}
\begin{algorithmic}
\STATE \textbf{INIT}: Initialize the weights $p_1, p_2,...p_N$ of all experts to $1/N$. \\
\FOR{ $t=1,2,\ldots,T$}
    \STATE Get the prediction $x_1,...,x_N$ from $N$ experts.
    \STATE Output 1 if $\sum_{i:x_i=1}p_i\geq\sum_{i:x_i=0}p_i$ otherwise output 0.
    \STATE receive the true value. If the $i$-th expert made a mistake, $p_i=p_i*\beta$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Randomized Multiplicative Weights Algorithms}
This algorithm works under the same assumption that the expert advices are all binary \cite{arora2012multiplicative}. While the prediction is random. The algorithm gives the prediction 1 with probability of $\gamma=\frac{\sum_{i:x_i=1}p_i}{\sum_i^N p_i}$ and 0 with probability of $1-\gamma$.


\subsection{Hedge Algorithm}

One of the well-known approaches for online prediction with expert advice is the Hedge algorithm \cite{DBLP:journals/jcss/FreundS97}, which can be viewed as a direct generalization of Littlestone and Warmuth's weighted majority algorithm~\cite{DBLP:journals/iandc/LittlestoneW94,littlestone1989weighted}. The working of Hedge algorithm is shown in Algorithm \ref{alg:hedge}

\begin{algorithm}[hptb]
\label{alg:hedge}
\caption{Hedge Algorithm}
\begin{algorithmic}
\STATE \textbf{INIT}: $\beta\in[0,1]$, initial weight vector $\w_1\in[0,1]^N$ with $\sum^N_{i=1}w_{1,i}=1$\\
\FOR{ $t=1,2,\ldots,T$}
    \STATE set distribution $\p_t=\frac{\w_t}{\sum^N_{i=1}w_{t,i}}$;
    \STATE Receive loss $\mathbf{\ell}_t\in[0,1]^N$ from environment;
    \STATE Suffer loss $\p_t^\top\mathbf{\ell}_t$;
    \STATE Update the new weight vector to $w_{t+1,i}=w_{t,i}\beta^{\ell_{t,i}}$\\
\ENDFOR
\end{algorithmic}
\end{algorithm}

The algorithm maintains a weight vector whose value at time $t$ is denoted $\w_t=(w_{t,1},\ldots,w_{t,N})$. At all times, all weights are nonnegative. All of the weights of the initial weight vector $\w_1$ must be nonnegative and sum to one, which can be considered as a prior over the set of experts. If it is believed that one expert performs the best, it is better to assign it the most weight. If no prior is known, it is better to set all the initial weights equally, i.e., $w_{1,i}=1/N$ for all $i$.  The algorithm uses the normalized distribution to make prediction, i.e., $\p_t={\w_t}/{\sum^N_{i=1}w_{t,i}}$. After the loss $\ell_t$ is disclosed, the weight vector $\w_t$ is updated using a multiplicative rule $w_{t+1,i}=w_{t,i}\beta^{\ell_{t,i}},\quad \beta\in[0,1]$, which implies that the weight of expert $i$ will exponentially decrease with the loss $\ell_{t,i}$.
In theory, the Hedge algorithm is proved to be Hannan consistent.

\if 0
Theoretically, for any sequence of loss vectors $\ell_1,\ell_2,\ldots,\ell_T$, and for any $i\in\{1,\ldots,N\}$, we have
\bqs
L_T\le \frac{\ln (1/\beta)}{1-\beta} L_{T,i} + \frac{\ln(1/w_{1,i})}{1-\beta}
\eqs
More generally, for any nonempty set $S\subseteq\{1,\ldots,N\}$, we have
\bqs
L_T\le \frac{\ln(1/\beta)}{1-\beta}\max_{i\in S}L_{T,i} + \frac{\ln(1/\sum_{i\in S}w_{1,i})}{1-\beta}
\eqs

More specifically, if the initial distribution is uniform and $\beta$ is set as $\frac{1}{1+\sqrt{2\ln N/T}}$, the per-round regret of Hedge is
\bqs
\frac{R_T}{T}= \frac{L_T}{T}-\min_i\frac{L_{T,i}}{T}\le \sqrt{\frac{2\ln N}{T}}+\frac{\ln N}{T}
\eqs
which implies that the Hedge algorithm is Hannan consistent.
\fi


%\subsubsection{Other Algorithms}

% add more subsubsections

\subsection{Other Algorithms}

Besides Hedge, there are some other algorithms for online prediction with expert advice under more challenging settings, including exponentially weighted average forecaster (EWAF) and Greedy Forecaster (GF)~\cite{DBLP:books/daglib/0016248}. We will mainly discuss EWAF, which is shown in Algorithm \ref{alg:ewaf}

\begin{algorithm}[hptb]
\caption{EWAF}
\label{alg:ewaf}
\begin{algorithmic}
\STATE \textbf{INIT}: a poll of experts $f_i,\quad i=1,\ldots,N$ and $L_{0,i}=0,\ i=1,\ldots,N$, and learning rate $\eta$ \\
\FOR{ $t=1,2,\ldots,T$}
    \STATE The environment chooses the next outcome $y_t$ and the expert advice $\{f_{t,i}\}$;
    \STATE The expert advice is revealed to the forecaster
    \STATE The forecaster chooses the prediction $\hat{p}_t=\frac{\sum^N_{i=1}\exp(-\eta L_{t-1,i})f_{t,i}}{\sum^N_{i=1}\exp(-\eta L_{t-1,i})}$
    \STATE The environment reveals the outcome $y_t$;
    \STATE The forecaster incurs loss $\ell(\hat{p}_t,y_t)$ and;
    \STATE Each expert incurs loss $\ell(f_{t,i},y_t)$
    \STATE The forecaster update the cumulative loss $L_{t,i}=L_{t-1,i}+\ell(f_{t,i},y_t)$
\ENDFOR
\end{algorithmic}
\end{algorithm}

The difference between EWAF and Hedge is that the loss in Hedge is the inner product between the distribution and the loss suffered by each expert, while for EWAF, the loss is between the prediction and the true label, which can be much more complex.

\if 0
Theoretically, if the loss function $\ell$ is convex in its first argument and it takes value in $[0,1]$ without loss of generality. For any $T$ and $\eta>0$, and for all any $y_1,\ldots,y_T$, the regret of the exponentially weighted average forecaster satisfies
\bqs
L_T-\min_i L_{T,i}\le \frac{\ln N}{\eta}+ {\eta N}{2}.
\eqs
Optimizing the upper bound suggests the choice $\eta =\sqrt{2\ln N/n}$ will result in  and upper bound $\sqrt{2T\ln T}$, which is $o(T)$ so that this algorithm is Hannan consistent. In addition, the introduction of loss function make that this algorithm can be used for many specific problems, like classification task.
\fi






\if 0 Sparse online learning is related to online feature selection since they both learn an efficient classifier for very high dimensional data. However, the sparse learning algorithms aim to minimize the $\ell$-1 regularized loss, while the feature selection algorithms are motivated to explicitly address the feature selection issue and thus impose a hard constraint on the number of non-zero elements in classifier. Because of these similarities, they share some common strategies such as truncation and projection. We will discuss it in the next section.
\fi












\if 0
\subsection{Online Learning with Concept Drift}
In a supervised learning scenario, the conditional distribution of the label $y_t$ given the input feature vector $\x_t$ may change over time, which makes it hard for the model leant on earlier data to make accurate predictions on new data. This phenomenon is termed as\emph{ Concept Drift}.

Although online learning is naturally better at addressing this problem compared with batch learning, special techniques are still required when designing online algorithms in concept drift environment. In literature, many surveys are available for a comprehensive introduction \cite{gama2014survey,vzliobaite2010learning,tsymbal2004problem}. Following, we will review the basic concepts and techniques in the topic online learning with concept drift.

The data distribution may change in two ways.
\begin{itemize}
\item \emph{Real Concept Drift.} The conditional distribution of class label given the feature distribution, $p(y|X)$, changes over time. This kind of drift is important since it affects the predictive decision.
\item \emph{Virtual Drift.} The distribution of features $P(X)$ changes over time but $p(y|X)$ is fixed. This kind of drift is not of key importance since it doesn't affect the decision function.
\end{itemize}

Based on the changing scale and time length, the concept drift problem can mainly be categorized into four classes,
 \begin{itemize}
\item  \emph{Sudden drift}. At certain time $t$, the old decision function $f(\x)$ is suddenly and totally replaced by a new function $g(\x)$.
\item \emph{Gradual drift}.  The old pattern is replaced by new pattern slowly over a long period. The weight of $f(\x)$ decreases and the weight of $g(\x)$ increases over time.
\item \emph{Incremental drift}.
 The incremental drift is similar to the gradual drift in that the pattern changes over a long time. But differently, it is not a replacement of two far away patterns, but an incremental change of the old pattern.
 \item \emph{Reoccurring contexts}. In the reoccurring contexts, previously active concept will reappear after some time.


  \end{itemize}

One of the biggest challenges for learning with concept drift is the trade-off between the effectiveness in detecting the drift and the robustness to noise. Specially, when $p(y|X)$ changes, the algorithm needs to distinguish if this is caused by noise or concept drift. If this is concept drift, the algorithm should react as soon as possible so that the online prediction accuracy does not degrade. If it is only noise, the model should stay stable. In order to be robust to noise, the algorithm should wait for many instances before it detects the drift. However, this may result in slow adaption to concept drift. Consequence, a good algorithm for learning with concept drift is required to handle this trade-off properly.

Based on when the adaptivity is switched on, The learning algorithms can be grouped into two types, \emph{trigger based} and \emph{evolving}. In a trigger based algorithm \cite{vzliobaite2009determining,su2008modeling,nishida2007detecting}, there is a change detector component that justifies if there is a concept drift happening based on data distribution, model parameters or output errors. When the change detector catches a big change, the algorithm switches on the adaptivity which may include discarding the old training data or model. Trigger based algorithms are good at dealing with a sudden drift. While in a evolving algorithm \cite{bifet2009new,delany2006comparison,karnick2008learning}, no implicit change detector exists. The most popular evolving technique classifier ensemble. The algorithm can learn several models and keep evaluating these models to estimate a proper weight for each model. And the final prediction is based on the weighted sum of the prediction of these models. By changing the weights of these ensembles, the algorithm can adapt to gradual drift.
\fi 

